D-Sempre: Learning Deep Semantic-Preserving Embeddings for User interests-Social Contents Modeling

Exponential growth of social media consumption demands effective user interests-social contents modeling for more personalized recommendation and social media summarization. However, due to the heterogeneous nature of social contents, traditional approaches lack the ability of capturing the hidden semantic correlations across these multi-modal data, which leads to semantic gaps between social content understanding and user interests. To effectively bridge the semantic gaps, we propose a novel deep learning framework for user interests-social contents modeling. We first mine and parse data, i.e. textual content, visual content, social context and social relation, from heterogeneous social media feeds. Then, we design a two-branch network to map the social contents and users into a same latent space. Particularly, the network is trained by a large margin objective that combines a cross-instance distance constraint with a within-instance semantic-preserving constraint in an end-to- end manner. At last, a Deep Semantic-Preserving Embedding (D-Sempre) is learned, and the ranking results can be given by calculating distances between social contents and users. To demonstrate the effectiveness of D-Sempre in user interests-social contents modeling, we construct a Twitter dataset and conduct extensive experiments on it. As a result, D-Sempre effectively integrates the multi-modal data from heterogeneous social media feeds and captures the hidden semantic correlations between users' interests and social contents.

==> ACM MM/acmmm17_version1.tex <==
\section{Introduction} \label{introduction}

\begin{figure}[!t]
	\centering
	\includegraphics[height=4.5cm, width=8.5cm]{figures/intro.jpg}
	\caption{}
	\label{intro}
\end{figure}
%%% background %%%%%%%%%%%%%%
The recent proliferation of social networks has revolutionized everyone's life, and its nature has gradually been shifted from the conventional user-centric networks such as Facebook(i.e. friendship based) to content-centric social networks such as Twitter, Printerest and Flickr. The development of content-centric social networks originates from users' emerging need - a pure interests-based social service to explore and collect interesting contents (such as images, videos and articles), through which to communicate with people who share similar interests. However, the traditional recommender systems, which attempt to capture the popularity of social items, are not designed to function effectively in this new era. Because a generally popular item does not necessarily mean it will be interested to a particular user, since interestingness is subjective and relevant to user's own taste.  
To generate better recommendations for users, researchers have turned to build personalized models to predict users' interestingness. While much effort have been made to generate more personalized social media recommendation, less progress has been made due to the following challenges: 

%%%% challenges %%%%%%%%%%%%%%
(1) Heterogeneous social media feeds are highly unstructured and lack direct representations. Previous works have primarily focused on the structured textual data, and the rich signals in visual content and the social contexts have been ignored. Some recent methods attempt to process these heterogeneous data, but they often perform separate processing and then simply combining them. The most recent work in \cite{Chen:2016:ACMMM} is the first attempt of using Deep Neural Network to directly take both high-dimensional sparse feature and images as input for integrate recommendation. However, the naive combination of visual content and user profile fails to capture the semantic correlation of user interests and social contents, and thus the recommendation performance is limited. Figure 1(a) gives an intuitive illustration of how the semantic gap impairs the recommendation performance. We use different color to represent different users, and each eclipse represents a hidden semantic space. It can be seen that, given a new item, the correlation among the three items (a new item and two items from two users) is not clear by considering the textual content, and is very close by considering the visual content. Thus, the recommender system will give an ambiguous matching result. 

(2) User-items interaction data are often too sparse and implicit. Users rarely provide ratings on items but rather give implicit feedback, which impairs the recommendation quality. 
Content-based filtering (CBF) recommends items based on a comparison between the contents of the items and a user profile \cite{Saveski:2014:RecSys, Balabanovic:1997:ACM}. However, when a user only rates a limited number of items, the limited content information cannot be generalized to discover the user's broader interests. 
Collaborative Filtering (CF)\cite{Su:2009:ACM} recommends items to users based on the items shared by other users with similar interests. However, CF also cannot achieve satisfied performance when the network is very sparse.
Figure 1(b) depicts an example of a recommender system, which consists of three users, four items and five hidden topics. In this example, user u1 liked item v1 and v2. user u2 liked item v3. Thus users u1 and u2 have no commonly liked items. This situation is a typical data sparsity problem (i.e., the known user-item actions are rare comparing with all the user-item pairs). In this situation, the existing CF approaches, e.g., PMF and CTR, cannot essentially recommend item v1 to user u2 because they cannot capture any relation between them. However, a good recommender system should recommend items v3 to user u1 and recommend item v1 and v2 to user u2, because in this example, users u1 and u2 are probably researchers on AI areas, and items v1, v2, and v3 are probably related to AI.

(3) The social media data has the ubiquitous cold-start
problem: most live items are newly generated and have never been seen in the training data. To tackle this, Chen \cite{Chen:2016:ACMMM} goes beyond modeling the interaction of user and item IDs that are sparse for new items, and models more dense interactions by examining the properties of the content itself as features. They follow the paradigm of factorization machines (FM), and transform the user-item interaction matrix to a set of feature vectors (model input) and a vector of interactions (target). We argue that such method is essentially a "shallow" model since it directly seek the resultant high-level features from user item matrix. When the matrix is very sparse, it will fail to find meaningful latent factors.


%%% our propose %%%%%%%%
In this paper, we propose a Bi-directional deep learning framework for the purpose of making personalized recommendation. The network consists of two sub-networks, which map a social media item and the user into a same latent semantic space, respectively. Therefore, the network achieves representations of both items and users, termed hybrid embedding hereafter, and this hybrid embedding are directly comparable to make decisions of recommendations. We use two items compared against one user, and learns the distance among them. Thus, the training data are triplets (user, positive item and negative item). Different from uniform sampling that is widely used for sampling negative instances. We adopt a time-aware negative sampling strategy, which improves the pairwise learning performance.

In order to bridge users' interests and social content, we incorporate social context and develop a large-margin objective to capture the semantic correlation between them. Specifically, the objective function combines the cross-view ranking constraints with within-view semantic preservation constraints. In the learned latent space, we want user with similar semantic liked items to be close to each other, so that to effectively capture the semantic correlations. Moreover, by integrate utilizing the heterogeneous social contents and contexts, although an new item has not been seen before, we can still infer a user's preference on new items based on their features (whose preferences have been learned during training). Consequently, the proposed scheme can help deal with the data sparse problem and the cold-start problem. 
The main contributions of this proposed scheme can be summarized into three-fold:

$\bullet$ We propose a novel deep learning framework that not only directly takes heterogeneous social media feeds as inputs, but also can be trained from end to end. This shall open a new avenue of deep learning research on heterogeneous information analyzing.

$\bullet$ We propose a Bi-directional learning model, using a pair of social media items compared against one user to learn their distances. We further adopt a time-aware negative sampling method, and thus achieves data that are more explicit and achieves superior performance. This strategy can be extended to other tasks that under implicit data situation. 

$\bullet$ We point out the important feature of hidden social context, and then train the network combined with semantic preservation constraints within each individual view, to effectively integrate contextual features and capture the semantic correlations for user interests modeling. The proposed learning framework is able to characterize the underlying structure of interrelationship among multiple model entities simultaneously. Consequently, it can help deal with the data sparsity and cold-start problem, which has potential usage value for multi-model learning. These constraints can also provide a useful regularization term for the cross-view matching task. 

\begin{figure*}
	\centering
	\includegraphics[scale=0.2]{figures/datamining.jpg}
	\caption{}
	\label{intro}
\end{figure*}
\section{Related Work}
Recommendation is a classic problem in Artificial Intelligence. Despite the fact that many works have studied the recommendation problem, they have primarily focused on the structured textual items such as book, movie, and music \cite{G.Adomavicius:2005:survey}. Typical technologies include content-based filtering collaborative filtering, and hybrid of both \cite{Pazzani:1999:CF}. However, it is difficult to directly adopt these technologies for content-centric social media recommendations, due to the highly unstructured heterogeneous social media feeds and highly sparse  user-image interaction data. Users rarely provide ratings on images but rather
give implicit feedback. 

To tackle this, existing works incorporate textual content into collaborative filtering models. Specifically, Chen et al. \cite{Chen:2012:SIGIR} transformed the traditional user-tweet interaction matrix to a
user-word matrix before applying matrix factorization. Following
the same idea, Feng et al. \cite{Feng:2013:WSDM} additionally modelled
the user-hashtag interaction, since hashtags are good topic
indicators. Hong et al. \cite{Hong:2013:WSDM} extended the Factorization Machines to jointly model user-tweet relations and the textual tweet generation process.
 
While much effort have been made to generate more personalized social media digests, the bottleneck of these purely content based methods comes from the semantic gap between user interests and social content understanding \cite{Jamali:2009:KDD, M.Jiang:2014:TKDE}. More recently, researches have been done to bridging the gap by capturing the social context. For example, Cui et al. \cite{Cui:2014:ACMMM} propose a regularized dual-factor regression
method based on matrix factorization to capture the social
attributes for recommendations. In \cite{Wu:2016:ACMMM}, the significance of affective features in shaping users' social media behaviors has been revealed. Similarly, Yang \cite{Yang:2016:AAAI} unveiled how users' emotional statuses influence each other and how users' positions in the social network affect their influential strength about emotion. Chen \cite{Chen:2016:ACMMM} shifted from the images' pixels to their context and propose a context-aware image tweet-modeling framework to mine and fuse contextual information to model the social media semantics. Moreover, the evolution of social media popularity trends has also been studied and incorporated in generating digests \cite{Wu:2016:TMMMM}. 



However, these methods ignore the visual content of items, instead, they focus solely on modeling users by discovering user profiles and behavior
patterns. Therefore, several recent works are trying to analyze the visual content and then aggregate the image-level knowledge for recommendation. An interesting technique to automatically select, rank and present social media images was proposed in \cite{McParlane:2014:CIKM}. In \cite{Rudinac:2011:ACMMM}, another approach that uses community-contributed images to create representative and diverse visual summaries is presented. A similar work has also been reported recently in \cite{Xu:2015:IUI}, in which the proposed approach can automatically select a set of representative images to generate a concise visual summary of a real-world event. However, the representations of visual content and users are still isolated due to semantic gap and the sparsity of user-image interactions.

Only a few recent work is concentrated on joint modeling of users and visual content for making recommendations \cite{Liu:2015:ACMMM, Liu:2014:ACMMM, Sang:2012:ACMMM}. Sang et al. \cite{Sang:2012:ACMMM} propose a topic sensitive model that concerns user preferences and user-uploaded images to
study users' influences in social networks. Liu et al. \cite{Liu:2014:ACMMM}
propose to recommend images by voting strategy according
to learnt social embedded image representations. Until
now, the existing methods often perform separate processing
of user information and image and then simply combining
them. A fully integrated solution is to be investigated.

%To alleviate the sparsity problem, matrix factorization based CF models have been proposed, such as the Singular Value Decomposition (SVD) [25], Weighted Matrix Factorization (WMF) [13], and the combination of probabilistic matrix factorization (PMF) [19] and topic models [31]. These models assume that the user-image matrix has a low-rank reconstruction by low-dimensional user and image features. We argue that such methods are essentially “shallow” models since they directly seek the resultant high-level features from user image matrix. When the matrix is very sparse, these methods will fail to find meaningful latent factors.


\section{The Proposed Scheme}
In this section, we present the proposed framework for social network recommendation. We first describe the data mining strategy from heterogeneous data sources in Section \ref{datamining}, and then illustrate the network structure we adopted in Section \ref{network}. The training strategy and objective are presented in Section \ref{training}, and finally we also introduce the data sampling method we utilized in Section \ref{datasampling}. Since our proposed model learns hybrid representations, it is well suitable for content-centric recommendation tasks. Considering Twitter is the most representative and popular social network, in this section we will take Twitter recommendation for an example to discuss on the utility of our proposed method. However, in general, the proposed framework can be used for any other social networks, e.g. Flickr, which is discussed in Section \ref{experiment}.

\subsection{Social media data mining and parsing strategy} \label{datamining}
We address the hybrid representations, i.e. simultaneous representations of both users and posts in a same latent space via deep learning approach. Given the fact that data sources on social network is heterogeneous, how to prepare the training data is not obvious. In this paper, both of the intrinsic content and extrinsic context of a post is utilized to generate post descriptors. Given a query user, his personal profile and social relation are considered for user representation. More details will be presented in the following.

\subsubsection{Mining data for social posts representation}
As we discussed in Section \ref{introduction}, the data from social network has the ubiquitous cold-start problem. To tackle this, we attempt to go beyond modeling the interaction between user and post IDs that are sparse for new data, and models more dense interactions by examining the properties of the content itself as features. To effectively represent the content of each post, we not only mine the intrinsic data of each post, but also the external data which may contain hidden context of the post itself. An example is shown in Figure 5(a), where the intrinsic visual content is straightforward, i.e. the raw image $I_{En}$ from the post. It has been demonstrated in [], that compared to the textual words of a tweet, hashtags exhibit stronger semantic ties to the post [21]. For example, in Figure 5(a), the hashtag $\sharp$EmTechDigital describes the topic and event of the post. Therefore, we use hashtag $H_{tag}$ to enhance the intrinsic textual content $T_{En}$.  Specifically, we follow [] to break up hashtags into component words by Microsoft's Word Breaker API2 e.g., $\sharp$EmTechDigital will be broken up as "EM", "Tech" and "Digital". We then combine such component words with text from post $T_{En}$ to form the hashtag enhanced text. 

Despite the intrinsic content, the external hidden context is another important feature. To provide context as well as to circumvent length limitations, Twitter users also embed shortened hyper links in their tweets. This suggests the external resource is the original context for such tweets, and thus a reliable source for capturing the posts' semantics. We thus extract the main textual content from the linked URLs. We further leverage Google inverse web search engine to obtain the hidden context from from the visual content.
For a query image, Google Reverse Image Search offers a "best guess" at a short text description. It can be seen as translating from a visual description to a semantic description. Thus, we send each raw image $I_{En}$ as a query to the Google Reverse Image Search, then utilize the "best guess", as image's semantic description. Consequently, the information we mined from a post $P$ can be described as follow:
\begin{equation}
{P_{\inf o}} = {I_{En}} + {T_{En}} + {H_{tag}} + Google({I_{En}}) + \alpha  \cdot URL
\end{equation}
where $\alpha$ is a indication term which is 1 if there exists a hyper link in post $p$, otherwise $\alpha$ is 0.

\subsubsection{Mining data for user representation}
Different from previous works that dominantly simply encode users by users' personal profile, e.g. user tags, gender, location and etc. We also consider the social relationship, which plays an important role in shaping users' hidden preference features.
As shown in Figure 5(b), given a query user $u$, we mine the user profile (user description and location) and her social relations (all of her followees). As they are all textual content, we generate descriptors by using the well-known
word2vector [22]. Specifically, all the mined information are converted to vectors and then vectors are clustered by k-means into 2000 semantic clusters.
Then, the bag-of-words approach works on these clusters. 
%Fig. 3 shows the distribution of clusters, where we observe the clusters have variant frequencies and bear topical polymerism to some degree. 
The 2000 semantic clusters are pre-computed. In the stage of training and testing, given a new query user, we can directly adopt the bag-of-words approach to generate the 2000-dimension feature vector for user representation.

\subsection{Network Architecture} \label{network}
The architecture of the proposed network is shown in Figure 3. It can be seen that, the network has two branches. Let $P$ and $U$ denote the collections of the social posts and users. $P$ and $U$ are first feed into the posts encoding module and user encoding module, respectively. Fully connected layers with 1024 hidden nodes are connected on top of each module to generate their own 1024-dimension feature vector representations, i.e. $V_u$ and $V_p$. The following two branches consists of fully connected layers with Rectified Linear Unit (ReLU) nonlinearities between them. L2 normalization is followed at the end of each branch. We use the inner product between any two vectors over the learned embedding space to measure similarity, which is equivalent to the Euclidean distance since the outputs of the two embeddings are L2-normalized. In the following, $d(\cdot)$ will denote the Euclidean distance between any two vectors in the embedded space. Many complicated distance calculating networks can be adopted herein, but we leave them for future exploration. We train parameters of each of the branch together with the parameters of the embedding layers in an end-to-end manner.

\subsubsection*{Social posts and Users encoding modules}
Given a tweet, we consider the data from two different domains, i.e. textual content (articles) and visual content (raw images). Instead of simply concatenate them together, we design a social posts encoding module to capture the correlations between these two different source data, and represent each post effectively. As illustrated in Figure 2, the social item encoding module consists of two branches. One part, takes raw images as input and follows with a convolutional neural network, which is shown in Figure 3. We do not build a very deep network in consideration of the trade off between performance and training time. The ConvNet consists of 5 convolution layers. It takes 224$\times$224 raw images as input, and outputs 2048-dimensional feature vector for visual content. The second part, takes texts as input and applies Word2Vec text encoding. Same with the first part, a fully connected layer with 2048 hidden nodes is followed to generated a 2048-dimension feature vector for textual content. Subsequently, they are concatenated into one vector and fed to a fully-connected to generate a 1024-dimension feature vector as the post representation $V_p$.

To encode the user information is more straightforward. Specifically, we first adopt Word2Vec to process data we mined from user domain to generate a 2000-dimension feature vector (it has been described in details in Section). Then, two fully connected layers are followed to output the 1024-dimension user representation $V_u$


\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.25]{figures/net_structure.jpg}
	\caption{}
	\label{intro}
\end{figure}



\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.2]{figures/CNN.jpg}
	\caption{}
	\label{intro}
\end{figure}

%We pre-train the ConvNet on the images in our training dataset with category labels. After pre-training, a 1024-way fully-connected layer is connected behind the last convolution layer. 

\subsection{Training Objective} \label{training}
Our training objective is a stochastic hinge loss based function that includes bidirectional outer-instance distance constraints, together with inner-instance semantic-preserving constraints.

\subsubsection{Bi-directional outer-instance distance constraints}
Given a user $u_i$, its set of matching samples, i.e. positive sample and negative sample are denoted as ${p_j}^ + $ and ${p_k}^ - $, respectively.
We want the distance between $u_i$ and each positive sample post ${p_j}^+$ to be smaller than the distance between $u_i$ and each negative sample post ${p_k}^-$ by some enforced margin $m$:
\begin{equation}
d({u_i},{p_j}^ + ) + m < d({u_i},{p_k}^ - )\;\;\;\forall \;{p_j}^ +  \in {P_i}^ + ,\;\forall \;{p_k}^ -  \in {P_i}^ - 
\end{equation}

Figure 4(a) gives us an intuitive illustration of an embedding space that satisfies the outer-instance matching property. That is, each user is closer to all circles of the same color (representing its corresponding posts) than to any circles of the other color. Similarly, for any circle (posts), the closest user has the same color. However, for the new image query (white square), the embedding space still gives an ambiguous matching result since both orange and green circles are very close to it (it has been discussed in Section \ref{introduction}). Driven by this important issue, a question arises: Can
we find a way to push semantically similar posts (same color circles) closer to each other, so that the above problem will be mitigated for the new generated embedding? To resolve this technical issues, we add a semantic preserving constraints to preserve the inner-instance structure.

\subsubsection{Inner-instance semantic-preserving constraints}
\begin{figure}[!t]
	\centering
	\includegraphics[height=3cm, width=8.5cm]{figures/structure.jpg}
	\caption{}
	\label{intro}
\end{figure}

Let $S$ represent a set of semantic clusters, and ${\rm N}{\{ {p_i}\} ^s}$ denotes a set of neighborhood posts of $p_i$ that belong to the same semantic cluster $s$. Then we want to enforce a margin of $m$ between ${\rm N}{\{ {p_i}\} ^s}$ and any point outside of $S$:

\begin{equation}
d({p_i},{p_j}) + m < d({p_i},{p_k})\;\;\forall \;{p_j} \in {\rm N}{\{ {p_i}\} ^s}
\end{equation}

In order to generate these semantic clusters, we first adopt word2Vec to convert all sources of the textual contents (including text from post ($T_{En}$), hashtag ($H_{tag}$), as well as textual content from URLs ($URL$) and Google search engine ($Google(I_{En})$)) to vectors. Then these vectors are clustered by K-means into 2000 semantic clusters. The 2000 semantic clusters are pre-generated. In the stage of training and testing, given a new query user, we can directly adopting the bag-of-words method to generate the 2000-dimension feature vector. As we can see from Figure 4(b), after we add the semantic-preserving constraints, the distances between the new query and the other two samples are much more discriminative in the new generated embedding space.
 
% Fig. 3 shows the distribution of clusters, where we observe the clusters have variant frequencies and bear topical polymerism to some degree. 
Consequently, we combine these two constraints into our training objective, the loss function is given by:
\begin{equation}
\begin{array}{l}
L(U,P) = \sum\limits_{i,j,k} {\max [0,m + d({u_i},{p_j}^ + ) - d({u_i},{p_k}^ - )]} \\
\;\;\;\;\;\;\;\;\;\;\;\;\;\; + \lambda \sum\limits_{i,j,k} {\max [0,m + d({p_i},{p_j}) - d({p_i},{p_k})]} 
\end{array}
\end{equation}
where $\lambda$ controls the importance of the structure-preserving terms. 

Last but not the least question is how to make recommendations for users. This is performed in the following steps. First, the representation of a given query user is generated, it can be calculated and stored in advance, or can be calculated in parallel to accelerate. Then, when feeding a set of posts, the representation of each post can be generated by the proposed social post encoding module. Third, distances are calculated among the posts and the user. Finally, K nearest neighboring posts having minimum distances are chosen as recommendations.

\section{Experiment} \label{experiment}
\subsection{Data sampling} \label{datasampling}
\subsubsection*{Triplet sampling}
Our loss involves all triplets consisting
of a target instance, a positive match, and a negative
match. Optimizing over all such triplets is computationally
infeasible. Therefore, we sample triplets within each minibatch
and optimize our loss function using SGD. 

There are two key issues to be solved
before applying the CDL.  Second,
how to prepare triplets as training data.

For each positive pair (i.e., a ground truth image-sentence pair, two neighboring images, or two neighboring sentences), we then find at most top K
violations of each relevant constraint (we use K = 50 in the
implementation, although most pairs have many fewer violations).

Theoretical guarantees of such a sampling strategy
have been discussed in [40], though not in the context of
deep learning. In our experiments, we observe convergence
within 30 epochs on average.

\subsubsection*{negtive sampling}
Since the input is a set of triplets in our proposed CDL, it
is desirable to generate a set of pairwise posts (a positive
sample and a negative sample) for each user. Positive posts
for users are often handy since users’ behavior data such
as “retweet” and “like” give such information explicitly.
However, negative images are not obvious [6]. In the literature of general recommender systems, uniform
sampling is most widely used for sampling nagative instances
due to its simplicity and acceptable performance [25]. Such
sampling strategy assumes that all non-retweeted posts are
equally weighted as negative instances (tweets disliked by
user u). However, an post is not “liked” by a user dose not necessarily indicate
the user is not interested in the post, but rather the user
never saw it. To address this, we propose a time-aware negative sampling strategy motivated by []. Our key assumption is that if a user acted on a post, she should also have read other posts that were posted in close temporal proximity to the acted post. Such tweets are then more likely to
be true negatives. Given a known post interaction rt, we sample the non-acted posts in proportion to the time interval between the post and rt; i.e., posts closer to rt have a higher chance of being selected. Our featured negative sampling method improves pairwise learning. We study its efficacy in Section 5.3.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}



\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}
% end the environment with {table*}, NOTE not {table}!




\appendix
%Appendix A
% This next section command marks the start of
% Appendix B, and does not continue the present hierarchy




==> acmmm17_version1.tex <==
\section{Introduction} \label{introduction}

\begin{figure}[!t]
	\centering
	\includegraphics[height=4.5cm, width=8.5cm]{figures/intro.jpg}
	\caption{}
	\label{intro}
\end{figure}
%%% background %%%%%%%%%%%%%%
The recent proliferation of social networks has revolutionized everyone's life, and its nature has gradually been shifted from the conventional user-centric networks such as Facebook(i.e. friendship based) to content-centric social networks such as Twitter, Printerest and Flickr. The development of content-centric social networks originates from users' emerging need - a pure interests-based social service to explore and collect interesting contents (such as images, videos and articles), through which to communicate with people who share similar interests. However, the traditional recommender systems, which attempt to capture the popularity of social items, are not designed to function effectively in this new era. Because a generally popular item does not necessarily mean it will be interested to a particular user, since interestingness is subjective and relevant to user's own taste.  
To generate better recommendations for users, researchers have turned to build personalized models to predict users' interestingness. While much effort have been made to generate more personalized social media recommendation, less progress has been made due to the following challenges: 

%%%% challenges %%%%%%%%%%%%%%
(1) Heterogeneous social media feeds are highly unstructured and lack direct representations. Previous works have primarily focused on the structured textual data, and the rich signals in visual content and the social contexts have been ignored. Some recent methods attempt to process these heterogeneous data, but they often perform separate processing and then simply combining them. The most recent work in \cite{Chen:2016:ACMMM} is the first attempt of using Deep Neural Network to directly take both high-dimensional sparse feature and images as input for integrate recommendation. However, the naive combination of visual content and user profile fails to capture the semantic correlation of user interests and social contents, and thus the recommendation performance is limited. Figure 1(a) gives an intuitive illustration of how the semantic gap impairs the recommendation performance. We use different color to represent different users, and each eclipse represents a hidden semantic space. It can be seen that, given a new item, the correlation among the three items (a new item and two items from two users) is not clear by considering the textual content, and is very close by considering the visual content. Thus, the recommender system will give an ambiguous matching result. 

(2) User-items interaction data are often too sparse and implicit. Users rarely provide ratings on items but rather give implicit feedback, which impairs the recommendation quality. 
Content-based filtering (CBF) recommends items based on a comparison between the contents of the items and a user profile \cite{Saveski:2014:RecSys, Balabanovic:1997:ACM}. However, when a user only rates a limited number of items, the limited content information cannot be generalized to discover the user's broader interests. 
Collaborative Filtering (CF)\cite{Su:2009:ACM} recommends items to users based on the items shared by other users with similar interests. However, CF also cannot achieve satisfied performance when the network is very sparse.
Figure 1(b) depicts an example of a recommender system, which consists of three users, four items and five hidden topics. In this example, user u1 liked item v1 and v2. user u2 liked item v3. Thus users u1 and u2 have no commonly liked items. This situation is a typical data sparsity problem (i.e., the known user-item actions are rare comparing with all the user-item pairs). In this situation, the existing CF approaches, e.g., PMF and CTR, cannot essentially recommend item v1 to user u2 because they cannot capture any relation between them. However, a good recommender system should recommend items v3 to user u1 and recommend item v1 and v2 to user u2, because in this example, users u1 and u2 are probably researchers on AI areas, and items v1, v2, and v3 are probably related to AI.

(3) The social media data has the ubiquitous cold-start
problem: most live items are newly generated and have never been seen in the training data. To tackle this, Chen \cite{Chen:2016:ACMMM} goes beyond modeling the interaction of user and item IDs that are sparse for new items, and models more dense interactions by examining the properties of the content itself as features. They follow the paradigm of factorization machines (FM), and transform the user-item interaction matrix to a set of feature vectors (model input) and a vector of interactions (target). We argue that such method is essentially a "shallow" model since it directly seek the resultant high-level features from user item matrix. When the matrix is very sparse, it will fail to find meaningful latent factors.


%%% our propose %%%%%%%%
In this paper, we propose a Bi-directional deep learning framework for the purpose of making personalized recommendation. The network consists of two sub-networks, which map a social media item and the user into a same latent semantic space, respectively. Therefore, the network achieves representations of both items and users, termed hybrid embedding hereafter, and this hybrid embedding are directly comparable to make decisions of recommendations. We use two items compared against one user, and learns the distance among them. Thus, the training data are triplets (user, positive item and negative item). Different from uniform sampling that is widely used for sampling negative instances. We adopt a time-aware negative sampling strategy, which improves the pairwise learning performance.

In order to bridge users' interests and social content, we incorporate social context and develop a large-margin objective to capture the semantic correlation between them. Specifically, the objective function combines the cross-view ranking constraints with within-view semantic preservation constraints. In the learned latent space, we want user with similar semantic liked items to be close to each other, so that to effectively capture the semantic correlations. Moreover, by integrate utilizing the heterogeneous social contents and contexts, although an new item has not been seen before, we can still infer a user's preference on new items based on their features (whose preferences have been learned during training). Consequently, the proposed scheme can help deal with the data sparse problem and the cold-start problem. 
The main contributions of this proposed scheme can be summarized into three-fold:

$\bullet$ We propose a novel deep learning framework that not only directly takes heterogeneous social media feeds as inputs, but also can be trained from end to end. This shall open a new avenue of deep learning research on heterogeneous information analyzing.

$\bullet$ We propose a Bi-directional learning model, using a pair of social media items compared against one user to learn their distances. We further adopt a time-aware negative sampling method, and thus achieves data that are more explicit and achieves superior performance. This strategy can be extended to other tasks that under implicit data situation. 

$\bullet$ We point out the important feature of hidden social context, and then train the network combined with semantic preservation constraints within each individual view, to effectively integrate contextual features and capture the semantic correlations for user interests modeling. The proposed learning framework is able to characterize the underlying structure of interrelationship among multiple model entities simultaneously. Consequently, it can help deal with the data sparsity and cold-start problem, which has potential usage value for multi-model learning. These constraints can also provide a useful regularization term for the cross-view matching task. 

\begin{figure*}
	\centering
	\includegraphics[scale=0.2]{figures/datamining.jpg}
	\caption{}
	\label{intro}
\end{figure*}
\section{Related Work}
Recommendation is a classic problem in Artificial Intelligence. Despite the fact that many works have studied the recommendation problem, they have primarily focused on the structured textual items such as book, movie, and music \cite{G.Adomavicius:2005:survey}. Typical technologies include content-based filtering collaborative filtering, and hybrid of both \cite{Pazzani:1999:CF}. However, it is difficult to directly adopt these technologies for content-centric social media recommendations, due to the highly unstructured heterogeneous social media feeds and highly sparse  user-image interaction data. Users rarely provide ratings on images but rather
give implicit feedback. 

To tackle this, existing works incorporate textual content into collaborative filtering models. Specifically, Chen et al. \cite{Chen:2012:SIGIR} transformed the traditional user-tweet interaction matrix to a
user-word matrix before applying matrix factorization. Following
the same idea, Feng et al. \cite{Feng:2013:WSDM} additionally modelled
the user-hashtag interaction, since hashtags are good topic
indicators. Hong et al. \cite{Hong:2013:WSDM} extended the Factorization Machines to jointly model user-tweet relations and the textual tweet generation process.
 
While much effort have been made to generate more personalized social media digests, the bottleneck of these purely content based methods comes from the semantic gap between user interests and social content understanding \cite{Jamali:2009:KDD, M.Jiang:2014:TKDE}. More recently, researches have been done to bridging the gap by capturing the social context. For example, Cui et al. \cite{Cui:2014:ACMMM} propose a regularized dual-factor regression
method based on matrix factorization to capture the social
attributes for recommendations. In \cite{Wu:2016:ACMMM}, the significance of affective features in shaping users' social media behaviors has been revealed. Similarly, Yang \cite{Yang:2016:AAAI} unveiled how users' emotional statuses influence each other and how users' positions in the social network affect their influential strength about emotion. Chen \cite{Chen:2016:ACMMM} shifted from the images' pixels to their context and propose a context-aware image tweet-modeling framework to mine and fuse contextual information to model the social media semantics. Moreover, the evolution of social media popularity trends has also been studied and incorporated in generating digests \cite{Wu:2016:TMMMM}. 



However, these methods ignore the visual content of items, instead, they focus solely on modeling users by discovering user profiles and behavior
patterns. Therefore, several recent works are trying to analyze the visual content and then aggregate the image-level knowledge for recommendation. An interesting technique to automatically select, rank and present social media images was proposed in \cite{McParlane:2014:CIKM}. In \cite{Rudinac:2011:ACMMM}, another approach that uses community-contributed images to create representative and diverse visual summaries is presented. A similar work has also been reported recently in \cite{Xu:2015:IUI}, in which the proposed approach can automatically select a set of representative images to generate a concise visual summary of a real-world event. However, the representations of visual content and users are still isolated due to semantic gap and the sparsity of user-image interactions.

Only a few recent work is concentrated on joint modeling of users and visual content for making recommendations \cite{Liu:2015:ACMMM, Liu:2014:ACMMM, Sang:2012:ACMMM}. Sang et al. \cite{Sang:2012:ACMMM} propose a topic sensitive model that concerns user preferences and user-uploaded images to
study users' influences in social networks. Liu et al. \cite{Liu:2014:ACMMM}
propose to recommend images by voting strategy according
to learnt social embedded image representations. Until
now, the existing methods often perform separate processing
of user information and image and then simply combining
them. A fully integrated solution is to be investigated.

%To alleviate the sparsity problem, matrix factorization based CF models have been proposed, such as the Singular Value Decomposition (SVD) [25], Weighted Matrix Factorization (WMF) [13], and the combination of probabilistic matrix factorization (PMF) [19] and topic models [31]. These models assume that the user-image matrix has a low-rank reconstruction by low-dimensional user and image features. We argue that such methods are essentially “shallow” models since they directly seek the resultant high-level features from user image matrix. When the matrix is very sparse, these methods will fail to find meaningful latent factors.


\section{The Proposed Scheme}
In this section, we present the proposed framework for social network recommendation. We first describe the data mining strategy from heterogeneous data sources in Section \ref{datamining}, and then illustrate the network structure we adopted in Section \ref{network}. The training strategy and objective are presented in Section \ref{training}, and finally we also introduce the data sampling method we utilized in Section \ref{datasampling}. Since our proposed model learns hybrid representations, it is well suitable for content-centric recommendation tasks. Considering Twitter is the most representative and popular social network, in this section we will take Twitter recommendation for an example to discuss on the utility of our proposed method. However, in general, the proposed framework can be used for any other social networks, e.g. Flickr, which is discussed in Section \ref{experiment}.

\subsection{Social media data mining and parsing strategy} \label{datamining}
We address the hybrid representations, i.e. simultaneous representations of both users and posts in a same latent space via deep learning approach. Given the fact that data sources on social network is heterogeneous, how to prepare the training data is not obvious. In this paper, both of the intrinsic content and extrinsic context of a post is utilized to generate post descriptors. Given a query user, his personal profile and social relation are considered for user representation. More details will be presented in the following.

\subsubsection{Mining data for social posts representation}
As we discussed in Section \ref{introduction}, the data from social network has the ubiquitous cold-start problem. To tackle this, we attempt to go beyond modeling the interaction between user and post IDs that are sparse for new data, and models more dense interactions by examining the properties of the content itself as features. To effectively represent the content of each post, we not only mine the intrinsic data of each post, but also the external data which may contain hidden context of the post itself. An example is shown in Figure 5(a), where the intrinsic visual content is straightforward, i.e. the raw image $I_{En}$ from the post. It has been demonstrated in [], that compared to the textual words of a tweet, hashtags exhibit stronger semantic ties to the post [21]. For example, in Figure 5(a), the hashtag $\sharp$EmTechDigital describes the topic and event of the post. Therefore, we use hashtag $H_{tag}$ to enhance the intrinsic textual content $T_{En}$.  Specifically, we follow [] to break up hashtags into component words by Microsoft's Word Breaker API2 e.g., $\sharp$EmTechDigital will be broken up as "EM", "Tech" and "Digital". We then combine such component words with text from post $T_{En}$ to form the hashtag enhanced text. 

Despite the intrinsic content, the external hidden context is another important feature. To provide context as well as to circumvent length limitations, Twitter users also embed shortened hyper links in their tweets. This suggests the external resource is the original context for such tweets, and thus a reliable source for capturing the posts' semantics. We thus extract the main textual content from the linked URLs. We further leverage Google inverse web search engine to obtain the hidden context from from the visual content.
For a query image, Google Reverse Image Search offers a "best guess" at a short text description. It can be seen as translating from a visual description to a semantic description. Thus, we send each raw image $I_{En}$ as a query to the Google Reverse Image Search, then utilize the "best guess", as image's semantic description. Consequently, the information we mined from a post $P$ can be described as follow:
\begin{equation}
{P_{\inf o}} = {I_{En}} + {T_{En}} + {H_{tag}} + Google({I_{En}}) + \alpha  \cdot URL
\end{equation}
where $\alpha$ is a indication term which is 1 if there exists a hyper link in post $p$, otherwise $\alpha$ is 0.

\subsubsection{Mining data for user representation}
Different from previous works that dominantly simply encode users by users' personal profile, e.g. user tags, gender, location and etc. We also consider the social relationship, which plays an important role in shaping users' hidden preference features.
As shown in Figure 5(b), given a query user $u$, we mine the user profile (user description and location) and her social relations (all of her followees). As they are all textual content, we generate descriptors by using the well-known
word2vector [22]. Specifically, all the mined information are converted to vectors and then vectors are clustered by k-means into 2000 semantic clusters.
Then, the bag-of-words approach works on these clusters. 
%Fig. 3 shows the distribution of clusters, where we observe the clusters have variant frequencies and bear topical polymerism to some degree. 
The 2000 semantic clusters are pre-computed. In the stage of training and testing, given a new query user, we can directly adopt the bag-of-words approach to generate the 2000-dimension feature vector for user representation.

\subsection{Network Architecture} \label{network}
The architecture of the proposed network is shown in Figure 3. It can be seen that, the network has two branches. Let $P$ and $U$ denote the collections of the social posts and users. $P$ and $U$ are first feed into the posts encoding module and user encoding module, respectively. Fully connected layers with 1024 hidden nodes are connected on top of each module to generate their own 1024-dimension feature vector representations, i.e. $V_u$ and $V_p$. The following two branches consists of fully connected layers with Rectified Linear Unit (ReLU) nonlinearities between them. L2 normalization is followed at the end of each branch. We use the inner product between any two vectors over the learned embedding space to measure similarity, which is equivalent to the Euclidean distance since the outputs of the two embeddings are L2-normalized. In the following, $d(\cdot)$ will denote the Euclidean distance between any two vectors in the embedded space. Many complicated distance calculating networks can be adopted herein, but we leave them for future exploration. We train parameters of each of the branch together with the parameters of the embedding layers in an end-to-end manner.

\subsubsection*{Social posts and Users encoding modules}
Given a tweet, we consider the data from two different domains, i.e. textual content (articles) and visual content (raw images). Instead of simply concatenate them together, we design a social posts encoding module to capture the correlations between these two different source data, and represent each post effectively. As illustrated in Figure 2, the social item encoding module consists of two branches. One part, takes raw images as input and follows with a convolutional neural network, which is shown in Figure 3. We do not build a very deep network in consideration of the trade off between performance and training time. The ConvNet consists of 5 convolution layers. It takes 224$\times$224 raw images as input, and outputs 2048-dimensional feature vector for visual content. The second part, takes texts as input and applies Word2Vec text encoding. Same with the first part, a fully connected layer with 2048 hidden nodes is followed to generated a 2048-dimension feature vector for textual content. Subsequently, they are concatenated into one vector and fed to a fully-connected to generate a 1024-dimension feature vector as the post representation $V_p$.

To encode the user information is more straightforward. Specifically, we first adopt Word2Vec to process data we mined from user domain to generate a 2000-dimension feature vector (it has been described in details in Section). Then, two fully connected layers are followed to output the 1024-dimension user representation $V_u$


\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.25]{figures/net_structure.jpg}
	\caption{}
	\label{intro}
\end{figure}



\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.2]{figures/CNN.jpg}
	\caption{}
	\label{intro}
\end{figure}

%We pre-train the ConvNet on the images in our training dataset with category labels. After pre-training, a 1024-way fully-connected layer is connected behind the last convolution layer. 

\subsection{Training Objective} \label{training}
Our training objective is a stochastic hinge loss based function that includes bidirectional outer-instance distance constraints, together with inner-instance semantic-preserving constraints.

\subsubsection{Bi-directional outer-instance distance constraints}
Given a user $u_i$, its set of matching samples, i.e. positive sample and negative sample are denoted as ${p_j}^ + $ and ${p_k}^ - $, respectively.
We want the distance between $u_i$ and each positive sample post ${p_j}^+$ to be smaller than the distance between $u_i$ and each negative sample post ${p_k}^-$ by some enforced margin $m$:
\begin{equation}
d({u_i},{p_j}^ + ) + m < d({u_i},{p_k}^ - )\;\;\;\forall \;{p_j}^ +  \in {P_i}^ + ,\;\forall \;{p_k}^ -  \in {P_i}^ - 
\end{equation}

Figure 4(a) gives us an intuitive illustration of an embedding space that satisfies the outer-instance matching property. That is, each user is closer to all circles of the same color (representing its corresponding posts) than to any circles of the other color. Similarly, for any circle (posts), the closest user has the same color. However, for the new image query (white square), the embedding space still gives an ambiguous matching result since both orange and green circles are very close to it (it has been discussed in Section \ref{introduction}). Driven by this important issue, a question arises: Can
we find a way to push semantically similar posts (same color circles) closer to each other, so that the above problem will be mitigated for the new generated embedding? To resolve this technical issues, we add a semantic preserving constraints to preserve the inner-instance structure.

\subsubsection{Inner-instance semantic-preserving constraints}
\begin{figure}[!t]
	\centering
	\includegraphics[height=3cm, width=8.5cm]{figures/structure.jpg}
	\caption{}
	\label{intro}
\end{figure}

Let $S$ represent a set of semantic clusters, and ${\rm N}{\{ {p_i}\} ^s}$ denotes a set of neighborhood posts of $p_i$ that belong to the same semantic cluster $s$. Then we want to enforce a margin of $m$ between ${\rm N}{\{ {p_i}\} ^s}$ and any point outside of $S$:

\begin{equation}
d({p_i},{p_j}) + m < d({p_i},{p_k})\;\;\forall \;{p_j} \in {\rm N}{\{ {p_i}\} ^s}
\end{equation}

In order to generate these semantic clusters, we first adopt word2Vec to convert all sources of the textual contents (including text from post ($T_{En}$), hashtag ($H_{tag}$), as well as textual content from URLs ($URL$) and Google search engine ($Google(I_{En})$)) to vectors. Then these vectors are clustered by K-means into 2000 semantic clusters. The 2000 semantic clusters are pre-generated. In the stage of training and testing, given a new query user, we can directly adopting the bag-of-words method to generate the 2000-dimension feature vector. As we can see from Figure 4(b), after we add the semantic-preserving constraints, the distances between the new query and the other two samples are much more discriminative in the new generated embedding space.
 
% Fig. 3 shows the distribution of clusters, where we observe the clusters have variant frequencies and bear topical polymerism to some degree. 
Consequently, we combine these two constraints into our training objective, the loss function is given by:
\begin{equation}
\begin{array}{l}
L(U,P) = \sum\limits_{i,j,k} {\max [0,m + d({u_i},{p_j}^ + ) - d({u_i},{p_k}^ - )]} \\
\;\;\;\;\;\;\;\;\;\;\;\;\;\; + \lambda \sum\limits_{i,j,k} {\max [0,m + d({p_i},{p_j}) - d({p_i},{p_k})]} 
\end{array}
\end{equation}
where $\lambda$ controls the importance of the structure-preserving terms. 

Last but not the least question is how to make recommendations for users. This is performed in the following steps. First, the representation of a given query user is generated, it can be calculated and stored in advance, or can be calculated in parallel to accelerate. Then, when feeding a set of posts, the representation of each post can be generated by the proposed social post encoding module. Third, distances are calculated among the posts and the user. Finally, K nearest neighboring posts having minimum distances are chosen as recommendations.

\section{Experiment} \label{experiment}
\subsection{Data sampling} \label{datasampling}
\subsubsection*{Triplet sampling}
Our loss involves all triplets consisting
of a target instance, a positive match, and a negative
match. Optimizing over all such triplets is computationally
infeasible. Therefore, we sample triplets within each minibatch
and optimize our loss function using SGD. 

There are two key issues to be solved
before applying the CDL.  Second,
how to prepare triplets as training data.

For each positive pair (i.e., a ground truth image-sentence pair, two neighboring images, or two neighboring sentences), we then find at most top K
violations of each relevant constraint (we use K = 50 in the
implementation, although most pairs have many fewer violations).

Theoretical guarantees of such a sampling strategy
have been discussed in [40], though not in the context of
deep learning. In our experiments, we observe convergence
within 30 epochs on average.

\subsubsection*{negtive sampling}
Since the input is a set of triplets in our proposed CDL, it
is desirable to generate a set of pairwise posts (a positive
sample and a negative sample) for each user. Positive posts
for users are often handy since users’ behavior data such
as “retweet” and “like” give such information explicitly.
However, negative images are not obvious [6]. In the literature of general recommender systems, uniform
sampling is most widely used for sampling nagative instances
due to its simplicity and acceptable performance [25]. Such
sampling strategy assumes that all non-retweeted posts are
equally weighted as negative instances (tweets disliked by
user u). However, an post is not “liked” by a user dose not necessarily indicate
the user is not interested in the post, but rather the user
never saw it. To address this, we propose a time-aware negative sampling strategy motivated by []. Our key assumption is that if a user acted on a post, she should also have read other posts that were posted in close temporal proximity to the acted post. Such tweets are then more likely to
be true negatives. Given a known post interaction rt, we sample the non-acted posts in proportion to the time interval between the post and rt; i.e., posts closer to rt have a higher chance of being selected. Our featured negative sampling method improves pairwise learning. We study its efficacy in Section 5.3.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}



\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}
% end the environment with {table*}, NOTE not {table}!




\appendix
%Appendix A
% This next section command marks the start of
% Appendix B, and does not continue the present hierarchy



